Neural Network Approximation

Neural Networks (NNs) are the method of choice for building learning algorithms. Their popularity stems from their empirical success on several challenging learning problems. However, most scholars agree that a convincing theoretical explanation for this success is still lacking. This article surveys the known approximation properties of the outputs of NNs with the aim of uncovering the properties that are not present in the more traditional methods of approximation used in numerical analysis. Comparisons are made with traditional approximation methods from the viewpoint of rate distortion. Another major component in the analysis of numerical approximation is the computational time needed to construct the approximation and this in turn is intimately connected with the stability of the approximation algorithm. So the stability of numerical approximation using NNs is a large part of the analysis put forward. The survey, for the most part, is concerned with NNs using the popular ReLU activation function. In this case, the outputs of the NNs are piecewise linear functions on rather complicated partitions of the domain of $f$ into cells that are convex polytopes. When the architecture of the NN is fixed and the parameters are allowed to vary, the set of output functions of the NN is a parameterized nonlinear manifold. It is shown that this manifold has certain space filling properties leading to an increased ability to approximate (better rate distortion) but at the expense of numerical stability. The space filling creates a challenge to the numerical method in finding best or good parameter choices when trying to approximate.

==> ActaNumerica_1_ ArXiv/macros.tex <==
%\usepackage{color}
%\usepackage{amsmath, amsthm}
%%\numberwithin{equation}{subsection}
%%\renewcommand{\theequation}{\thesubsection\arabic{equation}}
%
%\usepackage{amsfonts}
%\usepackage{amssymb}
\usepackage{graphicx}
%\usepackage{epsf}
%\usepackage{epsfig}
%\usepackage[normalem]{ulem}
%%\usepackage{enumitem}
%%\usepackage{wrapfig}
%%\usepackage[french]{babel}
%%\usepackage[applemac] {inputenc}
%%\usepackage[T1]{fontenc}
%\usepackage{showlabels}
%%\usepackage[usenames]{xcolor}
%%\usepackage{showkeys}
\usepackage[dvipsnames]{xcolor}
%
%
\newcommand{\ron}[1]{{#1}} 
\newcommand{\bguergana}[1]{{\color{red}{#1}}} 
\newcommand{\guergana}[1]{{\color{red}{#1}}} 
\newcommand{\simon}[1]{{\color{blue}{#1}}} 
\newcommand{\boris}[1]{{\color{purple}{#1}}} 
%
\def\vp{\varphi}
\def\<{\langle}
\def\>{\rangle}
\def\t{\tilde}
\def\i{\infty}
\def\e{\varepsilon}
\def\sm{\setminus}
\def\nl{\newline}
\def\o{\overline}
\def\wt{\widetilde}
\def\wh{\widehat}
\def\cT{{\cal T}}
\def\Z{{\mathbb Z}}
\def\cS{{\cal S}}
\def\cL{{\cal L}}
\def\cA{{\cal A}}
\def\cC{{\cal C}}
\def\cI{{\cal I}}
\def\cN{{\cal N}}
\def\cK{{\cal K}}
\def\cV{{\cal V}}
\def\cM{{\cal M}}
\def\cF{{\cal F}}
\def\cP{{\cal P}}
\def\cE{{\cal E}}
\def\cx{{\cal J}}
\def\cJ{{\cal }}
\def\cD{{\cal D}}
\def\cP{{\cal P}}
\def\cO{{\cal O}}
\def\cX{{\cal X}}
\def\R{\mathbb{R}}
\def\N{\mathbb{N}}
\def\C{\mathbb{C}}
\def\Relu{\mathrm{ReLU}}
	
\def\Up{\overline{\underline{\Upsilon}}}
%\newlength{\Sigmalength}
%\settowidth{\Sigmalength}{$\Sigma$}
%\def\bdSigma{\Sigma$\hspace{-\Sigmalength}\hspace{.07 ex}$\Sigma$\hspace{-\Sigmalength}\hspace{.07 ex}\vspace{-.15ex}$\Sigma}
%\newlength{\Upsilonlength}
%\settowidth{\Upsilonlength}{$\Upsilon$}
%\def\bdUpsilon{\Upsilon $\hspace{-\Upsilonlength}\hspace{.07 ex}$\Upsilon $\hspace{-\Upsilonlength}\hspace{.07 ex}\vspace{-.07ex}$\Upsilon}
%\def\bdUp{\Up$\hspace{-\Upsilonlength}\hspace{.015 ex}$\bdUpsilon}
%\def\bdUp{\Up $\hspace{-\Upsilonlength}\hspace{-.07 ex}$\bdUpsilon}

\newcommand{\be}{\begin{equation}}
\newcommand{\ee}{\end{equation}}
\newcommand{\gives}{\rightarrow}
\newcommand{\set}[1]{\left\{#1\right\} }
\newcommand{\mN}{\mathcal N}
\newcommand{\E}[1]{\mathbb E\left[#1\right]}
%
\newcommand\eref[1]{{\rm (\ref{#1})}}
\def\rnew{\color{red} }
\def\bnew{\color{blue} }

%%%%%%%%%%%%
% from Boris, I think
%%%%%%%%%%%%

\newcommand{\eg}{{\it e.g.}}
\newcommand{\ie}{{\it i.e.}}
\newcommand{\etc}{{\it  etc.}}
\newcommand{\cn}{\citeasnoun}
\newcommand{\ignore}[1]{}
\newcommand{\lr}[1]{\left(#1\right)}
\newcommand{\inprod}[2]{\left\langle#1,#2\right\rangle}
%
\newtheorem{theorem}{Theorem}[section]
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{proposition}[theorem]{Proposition} 
\newtheorem{remark}{Remark}[section] 

\newcommand{\abs}[1]{\left|#1\right|}
\newcommand{\norm}[1]{\left|\left|#1\right|\right|}



%
%% %%%%%%%%%%%%%%%%%%%%%%%%%
%% NOT USED:
%% %%%%%%%%%%%%%%%%%%%%%%%%%
%
%% \newcommand{\stkout}[1]{\ifmmode\text{\sout{\ensuremath{#1}}}\else\sout{#1}\fi}
%% %\numberwithin{equation}{section}
%% \def\rnew{\color{red} }
%% \definecolor{ID2}{rgb}{1.0, 0.2, 0.0}
%% \definecolor{ID}{rgb}{0.0, 0.0, 0.0}
%% %\definecolor{BH}{rgb}{0.0, 0.0, 1.0}
%% \definecolor{BH}{rgb}{0.0, 0.5, 0.3}
%% \def\anew{\color{blue}}
%% \newcommand{\snew}[1]{{\color{orange}#1}}
%% %%%%%%%%
%% \renewcommand{\baselinestretch}{1.15}
%% \newcommand{\lr}[1]{\left(#1\right)}
%% \hoffset=-0.3cm
%% %\voffset=-2cm
%% \textwidth=17cm
%% \textheight=23cm
%% \parindent=0 cm
%% \parskip=.2 cm
%% %
%% \usepackage{fullpage}
%% \def\nou{\overline{\underline{N}}}
%% \def\snou{\overline{\underline{n}}}
%
%% %%%%%%%%%%%%%%%%%%%%%%%%%
%
%% \numberwithin{equation}{section}
%% \def\RR{\rm \hbox{I\kern-.2em\hbox{R}}}
%% \def\NN{\rm \hbox{I\kern-.2em\hbox{N}}}
%% \def\ZZ{\rm {{\rm Z}\kern-.28em{\rm Z}}}
%% \def\CC{\rm \hbox{C\kern -.5em {\raise .32ex \hbox{$\scriptscriptstyle
%% |$}}\kern
%% -.22em{\raise .6ex \hbox{$\scriptscriptstyle |$}}\kern .4em}}
%
%% \def\Chi{\raise .3ex
%% \hbox{\large $\chi$}} \def\vp{\varphi}
%% \def\lsima{\hbox{\kern -.6em\raisebox{-1ex}{$~\stackrel{\textstyle<}{\sim}~$}}\kern -.4em}
%% \def\lsim{\hbox{\kern -.2em\raisebox{-1ex}{$~\stackrel{\textstyle<}{\sim}~$}}\kern -.2em}
%% \def\gsim{\hbox{\kern -.2em\raisebox{-1ex}{$~\stackrel{\textstyle>}{\sim}~$}}\kern -.2em}
%% \def\[{\Bigl [}
%% \def\]{\Bigr ]}
%% \def\({\Bigl (}
%% \def\){\Bigr )}
%% \def\[{\Bigl [}
%% \def\]{\Bigr ]}
%% \def\({\Bigl (}
%% \def\){\Bigr )}
%% \def\L{\pounds}
%% \def\span{\mathop{span}}
%% \renewcommand{\theequation}{\arabic{equation}}
%% \newcommand{\bea}{$$ \begin{array}{lll}}
%% \newcommand{\eea}{\end{array} $$}
%% \newcommand{\bi}{\begin{itemize}}
%% \newcommand{\ei}{\end{itemize}}
%% \newcommand{\iref}[1]{(\ref{#1})}
%% \newcommand{\eref}[1]{\eqref{#1}}
%% %\newtheorem{theorem}{Theorem}
%% \newtheorem{theorem}{Theorem}[section]     % changed by Simon
%% \newtheorem{remark}{Remark}[section]         % changed by Simon
%% \newtheorem{lemma}[theorem]{Lemma}
%% \newtheorem{proposition}[theorem]{Proposition} 
%% \newtheorem{corollary}[theorem]{Corollary}
%% \newtheorem{definition}{Definition}[section]  % changed by Simon
%% \newtheorem{notation}{Notation}[section]
%% \newtheorem{hypothese}{Hypoth{\`e}se}[section]
%% \newtheorem{propriete}{Propri{\'e}t{\'e}}[section]
%% \newtheorem{theo}{Th{\'e}or{\`e}me}[section]
%% \newtheorem{prop}{Proposition}
%% \newtheorem{lemm}{Lemme}[section]
%% \newtheorem{coro}{Corollaire}[section]
%
%
%%   \newcommand{\wnote}[1]{\marginpar{\tiny \textcolor{red}{WD: #1}}}
%%   \newcommand{\anote}[1]{\marginpar{\tiny \textcolor{blue}{AC: #1}}}
%  
%% %-------------------------  ingrid ------------------------------------------
%
%
%
%% %-------------------------  ricardo  %---------------------------------------
%
%% \def\Vb{\mathbb V}
%% \def\V{\mathbb V}
%% \def\E{\mathbb E}
%% \def\P{\mathbb P}
%% \def\N{\mathbb N}
%% \def\Sb{\mathbb S}
%% \def\na{\nabla}
%% \def\bq{\mathbf q}
%% \def\M{\mathcal M}
%
%
 \def\argmin{\mathop{\rm argmin}}
 \def\argmax{\mathop{\rm argmax}}
 \def\prob{\mathop{\rm prob}}
 \def\dist{\mathop{\rm dist}}
 \def\span{\mathop{\rm span}}
 \def\esssup{\mathop{\rm essssup}}
 
%
%% \def\anew{\color{blue}}
%
%% \newcommand{\cs}{\clubsuit}
%% \newcommand{\bI}{{\bf I}}
%% \newcommand{\bG}{{\bf G}}
%% \newcommand{\bS}{{\bf S}}
%% \newcommand{\bD}{{\bf D}}
%% \newcommand{\bA}{{\bf A}}
%% \newcommand{\bT}{{\bf T}}
%% \newcommand{\bX}{{\bf X}}
%
%% \newcommand{\bx}{{\bf x}}
%% \newcommand{\ba}{{\bf a}}
%% \newcommand{\bb}{{\bf b}}
%% \newcommand{\bw}{{\bf w}}
%% \newcommand{\bu}{{\bf u}}
%
%% %---  definitions for the estimator, triangulation, marking    -----------------%
%% \newcommand{\triak}[1][k]{\ensuremath{\mathcal{T}_{#1}} } 
%% \newcommand{\triai}[1][i]{\ensuremath{\mathcal{T}^{#1}} }
%% \newcommand{\Mk}[1][k]{\ensuremath{\mathcal{M}_{#1}} } 
%% \newcommand{\Nk}[1][k]{\ensuremath{\mathcal{N}_{#1}} } 
%% \newcommand{\Rk}[1][k]{\ensuremath{\mathcal{R}_{#1}} }
%% \newcommand{\jump}[1]{\left[\negthinspace\left[{#1}\right]\negthinspace\right]}
%
%% \newcommand{\mathscript}{\mathscr}
%% \newcommand{\est}{\ensuremath{\mathscr E}}
%% \newcommand{\estk}[1][k]{\ensuremath{\est_{#1}}}
%
%% \newcommand{\grids}{\ensuremath{\mathbb T}}
%% \newcommand{\As}{{\mathbb A}_s}
%% \newcommand{\Bs}{{\mathbb B}_s}
%
%% %--- variables and parameters -------------------------------------------------%
%
%% \newcommand{\eps}{\varepsilon}
%
%% %---  procedures    ------------------------------------------------------------%
%% \newcommand{\GREEDY}{\textsf{GREEDY}\xspace}
%% \newcommand{\SOLVE}{\textsf{SOLVE}\xspace}
%% \newcommand{\MARK}{\textsf{MARK}\xspace}
%% \newcommand{\REFINE}{\textsf{REFINE}\xspace}
%% \newcommand{\ESTIMATE}{\textsf{ESTIMATE}\xspace}
%% \newcommand{\MAKECON}{\textsf{MAKECONFORM}\xspace}
%% \newcommand{\REDUCEOSC}{\textsf{REDUCE\_OSC}\xspace}
%% \newcommand{\UPDATE}{\textsf{UPDATE}\xspace}
%% \newcommand{\OSC}{\textsf{OSC}\xspace}
%
%% %---  discrete solutions -------------------------------------------------------%
%% \newcommand{\uk}[1][k]{\ensuremath{U_{#1}}}
%% \newcommand{\ek}[1][k]{\ensuremath{e_{#1}}}
%% \newcommand{\Ek}[1][k]{\ensuremath{E_{#1}}}
%% \newcommand{\jk}[1][k]{\ensuremath{j_{#1}}}
%% \newcommand{\Jk}[1][k]{\ensuremath{J_{#1}}}
%
%% %---  commands %----------------------------------------------------------------%
%% \newcommand{\step}[1]{\noindent\raisebox{1.5pt}[10pt][0pt]{\tiny\framebox{$#1$}}\xspace}
%% \DeclareMathOperator*{\infimum}{inf\vphantom{p}}
%
%
%% \newcommand{\surr}{\bar{e}}
